On The Efficiency of Widely Linear Precoding and Symbol Extension in Cellular Uplink

We investigate Gaussian widely linear precoding known as improper Gaussian signaling for the cellular uplink with inter-cell interference, known as interference multiple access channel (IMAC). This transmission scheme provides extra degrees of freedom by treating the real and imaginary components of the complex Gaussian signal differently. Since current standards mainly utilize linear beamforming for waveform generation, we highlight the benefits of widely linear beamforming over multiple temporal dimensions (symbol extension in time) in the IMAC. This scheme achieves significantly higher information rates compared to conventional proper Gaussian signaling at the expense of extra complexity at the transmission phase. We study the sum-power minimization problem under rate constraints. This problem is a difference of concave functions (DC) program, hence, a non-convex problem. By numerical simulations, we observe the benefits of improper Gaussian signaling alongside symbol extension in power consumption for both single-antenna and multi-antenna base stations. Interestingly, we observe that at strong interference scenarios, the efficiency of improper Gaussian signaling outperforms conventional proper Gaussian signaling at low rate demands. Moreover, in such scenarios the sum-power required for achieving particular rate demands is significantly reduced.

==> reference.tex <==
@ARTICLE{Ying2011,
author={Ying-Chang Liang and Kwang-Cheng Chen and Li, G.Y. and Mahonen, P.},
journal={IEEE Transactions on Vehicular Technology},
title="{Cognitive radio networking and communications: an overview}",
year={2011},
volume={60},
number={7},
pages={3386-3407},
month={Sept},}
@ARTICLE{Geir2008,
author={Geirhofer, S. and Lang Tong and Sadler, B.M.},
journal={IEEE Journal on Selected Areas in Communications},
title="{Cognitive Medium Access: Constraining Interference Based on Experimental Models}",
year={2008},
volume={26},
number={1},
pages={95-105},
month={Jan},}
@ARTICLE{Devroye2006,
author={Devroye, N. and Mitran, P. and Tarokh, Vahid},
journal={IEEE Transactions on Information Theory},
title="{Achievable rates in cognitive radio channels}",
year={2006},
volume={52},
number={5},
pages={1813-1827},
month={May},}
@Article{Soheyl2016,
author={S. Gherekhloo and A. Chaaban and Chen Di and A. Sezgin},
journal={IEEE Transactions on Information Theory},
title="{(Sub-)Optimality of Treating Interference as Noise in the Cellular Uplink With Weak Interference}",
year={2016},
volume={62},
number={1},
pages={322-356},
month={Jan},}
@Article{Telatar1999,
  author    = {E. Telatar},
  title     = "{Capacity of multi-antenna Gaussian channels}",
  journal   = {European Transactions on Telecommunications, ETT
},
  year      = {1999},
  volume = {10},
number = {6},
month = {Nov.},
}
}
@Article{Larsson2008,
author = {E. G. Larsson and E. A. Jorswieck},
title = "{Competition Versus Cooperation on the MISO Interference Channel}",
journal = {IEEE Transactions on Communications},
year = {2008},
volume = {26},
number = {7},
month = {Sep.},
}

@Article{Neeser1993,
author = {F. D. Neeser and J. L. Massey},
title = "{Proper Complex Random Processes with Applications to Information Theory}",
journal = {IEEE Transactions on Information Theory},
year = {1993},
volume = {39},
number = {4},
month = {July},
}
@Article{Ho2012,
author = {Z. K. M. Ho and E. Jorswieck},
title = "{Improper Gaussian Signaling on the Two-User SISO Interference Channel}",
journal = {IEEE Transactions on Wireless Communications},
year = {2012},
volume = {11},
number = {9},
month = {Sep.},
}
@Article{Zeng2013,
author = { Y. Zeng and C. M. Yetis and E. Gunawan and Y.L. Guan and R. Zhang},
title = "{Transmit Optimization with Improper Gaussian Signaling for Interference Channels}",
journal = {IEEE Transactions on Signal Processing},
year = {2013},
volume = {61},
number = {11},
month = {June},
}

@Article{Jafar2009,
author = {V. Cadambe and S. A. Jafar and C. Wang},
title = "{Interference Alignment with Asymmetric Complex Signaling-Settling the Host-Madson Nosratinia Conjecture}",
journal = {IEEE Transactions on Information Theory},
year = {2010},
volume = {56},
number = {9},
month = {Sep.},
}

@Article{Sato1981,
author = {H. Sato},
title = "{The Capacity of the Gaussian Interference Channel Under Strong Interference}",
journal = {IEEE Transactions on Information Theory},
year = {1981},
volume = {27},
number = {6},
month = {Nov.},
}

@Article{Veravalli2009,
author = {V. S. Annapureddy and V. V. Veeravalli},
title = "{Gaussian Interference Networks: Sum Capacity in the Low-Interference Regime and New Outer Bounds on the Capacity Region}",
journal = {IEEE Transactions on Information Theory},
year = {2009},
volume = {55},
number = {7},
month = {July},
}

@Article{Zhang2010,
author = {R. Zhang and S.Cu},
title = "{Cooperative Interference Management with MISO Beamforming}",
journal = {IEEE Transactions on Signal Processing},
year = {2010},
volume = {58},
number = {10},
month = {Oct.},
}

@Book{Schreier2010,
author = {P. J. Schreier and L. L. Scharf},
title = "{Statistical Signal Processing of Complex-Valued Data: The Theory of Improper and Noncircular Signals}",
publisher = {Cambridge, U.K.: Cambridge Univ. Press},
}


@Book{Boyd2004,
author = { S. Boyd and L. Vandenberghe},
title = "{Convex Optimization}",
publisher = {Cambridge, U.K.: Cambridge Univ. Press},
}

@Book{Cover2006,
author = {T. Cover and J. Thomas},
title = "{Elements of Information theory}",
publisher = {New York: Wiley},
}

@Booklet{Grant2014,
title = "{The CVX Users' Guide}",
key = {Release 2.1},
author = {M. C. Grant and S. P. Boyd},
month = {Sep.},
year = {2014},
}

@Article{Laya2014,
author = {A. Laya and K. Wang and A. A. Widaa and J. A.-Zarate and J. Markendahl and L. Alonso},
title = "{Device-To-Device Communications And Small Cells: Eabling Spectrum Reuse For Dense Networks}",
journal = {IEEE Wireless Communication Magazine},
year = {2014},
month = {August},
}


@Article{Shang2007,
author = {X. Shang and G. Kramer and B. Chen},
title = "{A New Outer Bound and the Noisy-Interference Sum-Rate Capacity for Gaussian Interference Channels}",
journal = {IEEE Transactions on Information Theory},
year = {2009},
volume = {55},
number = {2},
month = {Feb.}
}

@Article{Geng2015,
author={C. Geng and N. Naderializadeh and A. S. Avestimehr and S. A. Jafar},
journal={IEEE Transactions on Information Theory},
title="{On the Optimality of Treating Interference as Noise}",
year={2015},
volume={61},
number={4},
pages={1753-1767},
month={April},}
@ARTICLE{Ottersten2014, 
author={Bjornson, E. and Jorswieck, E.A. and Debbah, M. and Ottersten, B.}, 
journal={IEEE Signal Processing Magazine}, 
title="{Multiobjective Signal Processing Optimization: The way to balance conflicting metrics in 5G systems}", 
year={2014}, 
month={Nov}, 
volume={31}, 
number={6}, 
pages={14-23}, 
}
@InProceedings{Schreier2015,
  Author         = {C. Lameiro and I. Santamaria and P. J. Schreier},
  Title          = "{Analysis of maximally improper signaling schemes for underlay cognitive radio networks}",
  BookTitle      = {IEEE International Conference on Communications (ICC), 2015},
  Address        = {London, UK},
  month          = {June},
  year           = 2015
}

@ARTICLE{Luo2010,
author={Zhi-Quan Luo and Wing-Kin Ma and So, A.M.-C. and Yinyu Ye and Zhang, Shuzhong},
journal={IEEE Signal Processing Magazine},
title="{Semidefinite Relaxation of Quadratic Optimization Problems}",
year={2010},
volume={27},
number={3},
pages={20-34},
month={May},}
@ARTICLE{Quan2006,
author={Zhi-Quan Luo and Wei Yu},
journal={IEEE Journal on Selected Areas in Communications},
title="{An introduction to convex optimization for communications and signal processing}",
year={2006},
volume={24},
number={8},
pages={1426-1438},
month={Aug},} 
@ARTICLE{Sidi2006,
author={Sidiropoulos, N.D. and Davidson, T.N. and Zhi-Quan Luo},
journal={IEEE Transactions on Signal Processing},
title="{Transmit beamforming for physical-layer multicasting}",
year={2006},
volume={54},
number={6},
pages={2239-2251},
month={June},}

@article{Quan2007,
author = {Zhi‐Quan  Luo and Nicholas D.  Sidiropoulos and Paul  Tseng and Shuzhong  Zhang},
title = "{Approximation Bounds for Quadratic Optimization with Homogeneous Quadratic Constraints}",
journal = {SIAM Journal on Optimization},
volume = {18},
number = {1},
pages = {1-28},
year = {2007},
} 

@ARTICLE{Dome2012,
author={A. De Domenico and E. Calvanese Strinati and M. G. Di Benedetto},
journal={IEEE Communications Surveys Tutorials},
title="{A Survey on MAC Strategies for Cognitive Radio Networks}",
year={2012},
volume={14},
number={1},
pages={21-44},
month={First Quarter},}  

@ARTICLE{Huang2010,
author={Y. Huang and D. P. Palomar},
journal={IEEE Transactions on Signal Processing},
title="{Rank-Constrained Separable Semidefinite Programming With Applications to Optimal Beamforming}",
year={2010},
volume={58},
number={2},
pages={664-678},
month={Feb},}
@ARTICLE{Dahrouj2011,
author={H. Dahrouj and W. Yu},
journal={IEEE Transactions on Communications},
title="{Multicell Interference Mitigation with Joint Beamforming and Common Message Decoding}",
year={2011},
volume={59},
number={8},
pages={2264-2273},
month={August},}

@inproceedings{chaaban2011interference,
  title="{Interference alignment and neutralization in a cognitive 3-user MAC-interference channel: degrees of freedom}",
  author={Chaaban, A. and Sezgin, A.},
  booktitle={12th CWIT},
  pages={26--29},
  year={2011},
}

@inproceedings{chaaban2011capacity,
  title="{Capacity results for a primary MAC in the presence of a cognitive radio}",
  author={Chaaban, A. and Sezgin, A.},
  booktitle={Proc. of GLOBECOM},
  pages={1--5},
  year={2011},
}
@InProceedings{ChaabanSezgin_EW2011,
  Author         = {A. Chaaban and A. Sezgin},
  Title          = "{On the capacity of the 2-user Gaussian MAC interfering with a P2P link}",
  BookTitle      = {European Wireless},
  Address        = {Vienna, Austria},
  month          = {27-29 Apr.},
  year           = 2011
}
@InProceedings{ZhuShangChenPoor,
  Author         = {Fangfang Zhu and Xiaohu Shang and Biao Chen and H.
                   Vincent Poor},
  Title          = "{On the capacity of multiple-access-Z-interference
                   channels}",
  BookTitle        = {Proc. of IEEE ICC},
  month = {June},
  year           = 2011
}
@InProceedings{BuehlerWunder,
  Author         = {J. B\"uhler and G. Wunder},
  Title          = "{Multiple access channel interfering with a point to point link: Linear deterministic sum capacity}",
  BookTitle      = {Proc. of IEEE ICC},
  Address        = {Ottawa, Canada},
  year           = {2012},
}
@book{Poor1994,
 author = {Poor, H. Vincent},
 title = "{An Introduction to Signal Detection and Estimation (2Nd Ed.)}",
 year = {1994},
 isbn = {0-387-94173-8},
 publisher = {Springer-Verlag New York, Inc.},
 address = {New York, NY, USA},
}   

@INPROCEEDINGS{KariminezhadICC2017, 
author={A. Kariminezhad and A. Sezgin and M. Pesavento}, 
booktitle={2017 IEEE International Conference on Communications (ICC)}, 
title="{Power efficiency of improper signaling in MIMO full-duplex relaying for K-user interference networks}", 
year={2017}, 
pages={1-6}, 
month={May},}

